Combining Query Performance Predictors: A Reproducibility Study

A large number of approaches to Query Performance Prediction (QPP) have been proposed over the last two decades. As early as 2009, Hauff et al. [28] explored whether different QPP methods may be combined to improve prediction quality. Since then, significant research has been done both on QPP approaches, as well as their evaluation. This study revisits Hauff et al.s work to assess the reproducibility of their findings in the light of new prediction methods, evaluation metrics, and datasets. We expand the scope of the earlier investigation by: (i) considering post-retrieval methods, including supervised neural techniques (only pre-retrieval techniques were studied in [28]); (ii) using sMARE for evaluation, in addition to the traditional correlation coefficients and RMSE; and (iii) experimenting with additional datasets (Clueweb09B and TREC DL). Our results largely support previous claims, but we also present several interesting findings. We interpret these findings by taking a more nuanced look at the correlation between QPP methods, examining whether they capture diverse information or rely on overlapping factors.

==> dim.tex <==
% * WT10g and or Gov2 te result bar kora
% * Neural network diye ei indd. QPP diye AP predict kora (MSMARCO dev queries)
% * rank vs QPP score ta plot korle na na rokom method er jonyo na na rokom hoy, --- graph gulo dekhe jodi kichu mathay ashe eta ota try korar.. Ami eta initially Sir ke dekhiyechilam... 
% * Future work: Why is CW09b so messed up?
% * Try weighted-fusion techniques?
% * Explore adjusted rho

% Following from the above, is there a relationship in the performance patterns of different QP predictors, both within and between pre-retrieval and post-retrieval categories?
>>> QPP method gulo cluster kore dekha, let's run it on MsMarco dev Qs
% \textcolor{red}{eta future work e?}Specifically, can correlations or dependencies be identified that might shed light on how these predictors complement or overlap in their effectiveness across various datasets?

% 3. notun bacha der diye ei kaaj tar extension --- aaro aaro method aaro aaro dataset, kendall, rho --ghete jabar halka chance toh achei...


==> ecir25/TODO.tex <==
\begin{itemize}

%\item \textbf{CHANGE THE TITLE OF THE PAPER?}
%\item Section 4: Name change to \text{Results}.
%\item \red{\textbf{Table 2 er incomplte caption.} + Why is LOO required for sMARE??}
  
% \item As the values of the fused models have changed, check the \%-imp. cell for inconsistencies.

% \item \textbf{\textcolor{red}{Section 3 ``Retrieval settings and evaluations'' je je evaluation techniques use kora hoyeche ($\rho$, $\tau$, $sMARE$, $RMSE$), sei gulo bola.. tahole ar prottek table e repeat korte hobe na.}}

\item\textcolor{green}{MM} Abstract er inote er content ta baad to?

  MM: arektu results + analysis ta dekhe nie ei dabi ta koto jordar bhabe
  kora jay bujhe nie decision newa hoy?

%\item\textcolor{green}{MM?} Table 2 er explanation ta bhalo kore review kora.

%\item\textcolor{green}{MM?} Figure 2 er explanation.

%\item \textcolor{green}{MM?} Table 2 te amader $\rho$ gulor CI bhorti kora.


% \item\textcolor{blue}{SD?} Conclusion and Future Work
% \item\textcolor{red}{SS} LARs ek line
% \item\textcolor{red}{SS} table e E-net, .. short form bolchi mention that too
\item\textcolor{red}{SS} code gulo upload
%\item\textcolor{red}{SS} LARs e keno result bhalo aschena -- reason ta bhalo peyechi.. efron et al. (annals of stat 04) er detail discussion by weisberg  
% apatoto add kore dewa hok;
%SS 
% \item Note that, for OLS and Lars-CV, the $\rho$ and \emph{RMSE} values calculated in \cite{hauff2009combination} are not directly comparable, as they used 19 predictors while we use 10 selected predictors.

% :: shudhu 'selected' bolle tushto hobe?

% \item Sec 4 prochur bar dataset k refer korchhe. amra jehetu identifier byabohar korchhi e, pati {RB, CW, DL} byabohar korle jaiga bachto, kono confusion hote pare ete Table 1-a agei bole dile?

\end{itemize}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> ecir25/analysis.bck.tex <==
\section{Results and analysis} \label{sec:analysis}

\input{tabdefs/pre-ret}

\para{Reproducing results from \cite{hauff2009combination}}
%\inote{Naam ta
%  odd lagche: eta better?}%
As a validation check, we first repeat Hauff et al.'s experiments (with a
selected subset of the pre-retrieval predictors) on the TREC 678 topics (see Table~\ref{tab:datastats}).
Our results are presented in Table~\ref{tab:pre-ret-reprod-table}. We note
that our $\rho$ values are generally higher than those reported by Hauff et
al. Following their suggestion, we include the 95\% confidence interval
(CI) for the observed $\rho$ values. For two predictors (\texttt{AvP},
\texttt{AvNP}), the CIs (highlighted) are non-overlapping; since the
corresponding $\rho$s are fairly low on an absolute scale, we have not looked
more carefully into this difference. For \texttt{AvgSCQ} the difference
(underlined) appears numerically substantial, but is not, in fact,
statistically significant. Of greater concern is the noticeable difference
in $\rho$ for \texttt{AvgIDF} (highlighted). Strictly speaking, however, for
this predictor also, the corresponding CIs do overlap. Additionally, the
RMSE values that we obtain are all very close to those reported in
\cite{hauff2009combination}. We are able to conclude, therefore, that the
high-level summary of the results in Table~\ref{tab:pre-ret-reprod-table}
(that \texttt{MaxIDF}, \texttt{AvgIDF}, \texttt{AvgVAR} and \texttt{MaxVAR}
provide the best predictions, both in terms of $\rho$ and \emph{RMSE}) matches
the findings as in \cite{hauff2009combination}.

The second half of Table~\ref{tab:pre-ret-reprod-table} compares the combined models from our implementation with those reported by Hauff et al. 
We observe that the correlations, particularly in terms of Pearson's $\rho$, for the combined approaches (reported in~\cite{hauff2009combination}, Table 5) are somewhat higher than those from our implementation\footnote{Note that, the combinations in~\cite{hauff2009combination} were performed using 19 pre-retrieval predictors, whereas our fused results combine 10 of the best-selected predictors from their set.}.
% However, the \emph{RMSE} of the reproduced models are better than those reported in~\cite{hauff2009combination}.
However, we can see a slight improvement in terms of rank-correlation $\tau$ and \emph{sMARE}.
Overall, our observations from Table~\ref{tab:pre-ret-reprod-table} indicate that the improvements across all the evaluation measures are negligible.
This observation contrasts with the findings reported by Hauff et al. which states that ``\emph{Independent of the quality of the predictors, r increases as more predictors are added to the model}'' (see~\cite{hauff2009combination}, Figure 2).
Notably, their paper does not provide any justification for this surprising behaviour. 
In contrast, we offer an explanation for the differing results later in this section.
\mynote{TODO: Check the above para carefully.}

%\input{tabdefs/reg-pre}
\input{tabdefs/pre-combined}
%\input{tabdefs/post-ret}
%\input{tabdefs/reg-post}
\input{tabdefs/post-combined}
\input{figs/heatmap}
\input{figs/heatmap_pre_post}

\para{Pre-retrieval predictors on additional collections}
\itodo{CIs, significance tests for Tables 2, 3}
Table~\ref{tab:pre-ret-combined-table} presents the pre-retrieval QPP results across
three datasets in terms of Kendall's $\tau$, Pearson's $\rho$, \emph{sMARE}, and
\emph{RMSE}. The results for TREC DL are clearly in agreement with the
summary for Table~\ref{tab:pre-ret-reprod-table}: once again,
\texttt{MaxIDF}, \texttt{AvgIDF}, \texttt{MaxVAR}, and \texttt{AvgVAR}
appear to be the best performing predictors in terms of all metrics. This
observation mostly holds for TREC Robust as well, where \texttt{MaxSCQ}
also emerges as a promising measure, outperforming \texttt{MaxIDF} and
\texttt{AvgIDF} on two of the four metrics (these are underlined in
Table~\ref{tab:pre-ret-combined-table}). CW09B presents the most confusing
picture: there is little variation in the \emph{RMSE} values across all
methods; to a lesser extent, the same holds true for \emph{sMARE}. Overall,
\texttt{MaxSCQ} seems to deliver the best results, even though the
\texttt{IDF} and \texttt{VAR} variants also perform reasonably well.

\para{Results for post-retrieval predictors.}
The post-retrieval predictor results, shown in Table~\ref{tab:post-ret-combined-table}, reveal a clear distinction in performance between supervised and unsupervised methods, with \texttt{qppBERT-PL} performing best overall. For example, for TREC Robust queries, the best-performing unsupervised approach is \texttt{UEF-WIG}, with an \emph{RMSE} score of $0.1924$, whereas for supervised neural QP predictors, \emph{RMSE} of \texttt{qppBERT-PL} is $0.1632$. 
%The results for post-retrieval predictors are shown in Table~\ref{tab:post-ret-table}, where a clear distinction in performance can be observed between supervised and unsupervised approaches. 
%On the other hand, for post-retrieval based QPP approaches a clear distinction between the supervised and unsupervised approaches ca be made. 
%\texttt{qppBERT-PL} is the best-performing prediction approach in Table~\ref{tab:post-ret-table}.
Table~\ref{tab:pre-ret-reprod-table} presents the pre-retrieval results for TREC 678 ($150$ queries) using a leave-one-out approach, where $\rho$ (Hauff et al.) and \emph{RMSE} (Hauff et al.) refer to the actual values of $\rho$ and \emph{RMSE} as reported in~\cite{hauff2009combination}. 
To address \textbf{RQ-1}, the lower half of the Table~\ref{tab:pre-ret-reprod-table} reports
%we report (second half of Table~\ref{tab:pre-ret-reprod-table})
penalized regression values combining all pre-retrieval QP predictors as in Table~\ref{tab:pre-ret-combined-table}, where no substantial increase is observed in terms of either correlation or \emph{RMSE}, when comparing individual QPP measures with the combined approach. For instance, the \emph{RMSE} value decreases marginally from $0.1674$ (\texttt{AvgIDF}) to $0.1641$, and Pearson's $\rho$ increases slightly from $0.6283$ (\texttt{AvgIDF}) to $0.6398$ (Lars-CV).
This observation stands valid also for a recent dataset, such as TREC DL which answers to \textbf{RQ-1}.
%In the second row, we also report the penalized regression values combining all QP predictors. 
%Noticeably, when comparing individual QPP measures with the combined ones, there is no significant increase in correlation or \emph{RMSE}. 

Subsequently, we present the penalized regression results for TREC Robust, CW09B, and TREC DL and compare with the pre-retrieval results. Notably, combining pre-retrieval predictors does not improve results on the TREC Robust collection, and in CW09B and TREC DL collections, a decrease in correlation measures is observed. For example, for CW09B, Pearson's $\rho$ decreases from $0.2914$ (\texttt{MaxSCQ}) to $0.1763$ (Ridge-CV), and the \emph{sMARE}, \emph{RMSE} scores increase from $0.2660$ (\texttt{MaxIDF}) and $0.1625$ (\texttt{MaxSCQ}) to $0.2857$ (OLS) and $0.1661$ (E-Net-CV) respectively.
%. On the other hand, \textcolor{red}{we see a decrease} in correlation measure for ClueWeb09B and TREC-DL collections. 
To address \textbf{RQ-2}, Table~\ref{tab:post-ret-combined-table} reports 
%we report 
the combination of the post-retrieval based QPP methods across all three datasets. %in Table~\ref{tab:regr-post-ret-table}. 
For post-retrieval, the best-performing QPP method is \texttt{qppBERT-PL}, while \texttt{MaxIDF} leads among pre-retrieval methods. In TREC Robust, notable improvements are seen in $\tau$, $\rho$, and \emph{RMSE}. The \emph{RMSE} score declines significantly from $0.1632$ (\texttt{qppBERT-PL}) to $0.1378$ (LASSO-CV), with a \emph{p-value} of $0.0360$.
For significance, we compare \emph{p-value} with the best-performing QP predictors; however, no significant improvements are observed in other datasets, namely CW09B and TREC DL.
%For post-retrieval, method, the best performing QPP method is \emph{qPPBERT-PL} and \emph{MaxIDF} is for pre-retreival method. For, TREC Robust collection, we see a jump in terms of $\tau$, $\rho$ and RMSE values improve significantly. To compare, the \emph{p-value}, we compare with the best performing QP predictors. However, we do not a see significant improvement in other datasets, ClueWeb09B, and TREC-DL.  

% \emph{Analysis and observation}:
\para{Analysis}
To gain deeper insights into the penalized regression results, we compute Kendall's $\tau$ and Pearson's $\rho$ among the QP predictors. Figure~\ref{fig:heatmap} presents the correlation coefficients across QPP approaches across all three collections. Some QPP methods exhibit negative correlations; for instance, %We observe that some of the QPP methods are negatively correlated. For example, 
in the TREC DL collection, Pearson's $\rho$, Kendall's $\tau$ between \texttt{SumSCQ} and \texttt{AvgIDF} are $-0.5349$, and $-0.2878$, respectively. A similar pattern appears in CW09B, where \texttt{AvP} and \texttt{AvNP} are negatively correlated with \texttt{SumSCQ}. However, for TREC 678 queries, we observe no significant negative correlations among predictors, which we attribute as one reason why combining pre-retrieval QPP approaches does not enhance performance and may even reduce it. For the TREC collection, we also validate our correlation coefficients with those reported in~\cite{hauff_dissertation}, observing similar results for TREC 678 queries. 

%On combining these predictors using diffre

Interestingly, when comparing pre and post QP predictors, we find that \texttt{MaxIDF} and \texttt{AvgIDF}, despite their simplicity, perform similarly to unsupervised post-retrieval approaches in terms of \emph{RMSE} across the three datasets. In CW09B, \texttt{MaxIDF} even performs comparably to neural QPP approaches with respect to \emph{sMARE}.
%of \texttt{MaxIDF} is even comparable to neural QPP approaches in terms of \emph{sMARE}. 

% \textbf{RQ-1} On combining different QPP predictors, do we get a better predictor with respect to post-retrieval QPP approaches? Are the trends across these two datasets different? If so, why are we observing different results?




% \textbf{RQ-2} How effective is this result in comparison to pre-retrieval QPP approaches? Why are we getting a different trend on these two specific category of QPP approaches? Do we have an explanation for this?

%If we compare pre-retrieval QPP approaches with post-retrieval predictors, one clear distinction emerges. \texttt{MaxIDF} and \texttt{AvgIDF}, despite their simplicity, perform similarly to unsupervised post-retrieval approaches in terms of \emph{RMSE} across the three datasets.



% \textbf{RQ-3}
% In the literature of QPP, generally a correlation measure between the predicted AP (using QPP) and the actual AP is computed to quantify how well a QPP method is performing. As mentioned in the 

% \textbf{RQ-4}


\textcolor{red}{fusion er beparta, passing note e we can mention
A wide variation of fusion based techniques are used to combine different QPP approaches.}

\begin{comment}
    
Diversity between the QPP approaches? 

\textcolor{red}{fusion er beparta, passing note e we can mention
A wide variation of fusion based techniques are used to combine different QPP approaches.}


We observe an increase in RMSE scores with the COMBSUM based fusion technique. This motivates us to linearly combine QPP approaches. 
Why COMBSUM is performing better than all the fusion approaches? 
--- Linearly combining helps.. as we can see from the empirical results of LASSO and ...

\end{comment}
%*** Effect of channging the parameter $C$ in SVR. 
%\mynote{correlation between QPP methods?}

\mynote{table for only unsupervised approaches?}

%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "main"
%%% End:


==> ecir25/analysis2.tex <==
\input{figs/heatmap}
\section{Discussion} \label{sec:discussion}
% Query performance predictors aim to estimate expected retrieval performance in terms of AP; that is, for a given query and a retrieval model, the predictor estimates the average precision that a user is likely to experience.
% For all topics within a specific topic set (e.g., TREC Robust), correlations (e.g., Pearson's $\rho$ or Kendall's $\tau$) are calculated between each of the predicted AP scores and the actual observed AP scores; a high correlation indicates a better prediction by that predictor.
% The performance metrics reported in Table~\ref{tab:pre-ret-combined-table} and~\ref{tab:post-ret-combined-table} are based on those correlations.
Since the inception of research on performance prediction, efforts have primarily focused on enhancing predictors to make the prediction process more robust.
However, the relationships between different predictors have received limited attention.
Notably, only in~\cite{hauff_thesis} was this relationship explored, where the author reported Kendall's $\tau$ among a set of pre-retrieval predictors (see Tables 2.3 and 2.6 in~\cite{hauff_thesis}).

Building on this foundation, we investigate the behavior of combined predictors to gain deeper insights into the results.
Specifically, we compute the pairwise intra-predictor similarities (in terms of per-query $\rho$) to identify the underlying reasons for performance variations\footnote{We observe similar trends with respect to the $\tau$. Hence, the correlations based on $\rho$ is only reported in this paper due to space constraints. For the TREC collection, we also validate our correlation coefficients with those reported in~\cite{hauff_dissertation}, observing similar results for TREC 678 queries. }.
% This analysis aims to unravel how different predictors interact and contribute to overall predictive accuracy.
%
%
Figure~\ref{fig:heatmap} presents the pairwise $\rho$ values as a heatmap for each collections across prediction approaches. 
The figure reveals several surprising behaviors in the relationships between predictors.
Notably, we observe a high correlation ($\rho > 0.7$) among the \texttt{IDF} variants, \texttt{VAR} variants, collection-based specificity methods, and the polysemy-based approaches (\texttt{AvP} and \texttt{AvNP}) across all datasets when using pre-retrieval methods.
Overall, the correlation among the pre-retrieval predictors are seen to be moderate to high with the exception of \texttt{SumSCQ} and \texttt{SumVAR}, which do not correlate well with the other predictors.
However, their intra-correlation is notably strong, reaching a peak of $0.94$ in the case of CW09B.

In contrast, post-retrieval predictors generally show \emph{lower} intra-correlation.
Among these, only the \texttt{UEF} variants display moderate to high correlation with each other.
Neural methods, particularly \texttt{NeuralQPP}, \texttt{qppBERT-PL}, \texttt{Deep-QPP}, and \texttt{BERT-QPP}, demonstrate varied correlation behavior; for collections with fewer training queries (e.g., TREC Robust and CW09B), these methods show negligible correlation, while their correlations increase with the availability of more training data, as observed with the TREC DL collection ($\rho > 0.5$).

Further, we observe nearly zero to negative intra-predictor correlations, particularly among the pre-retrieval predictors in the TREC DL collection.
For example, in the TREC DL collection,correlations between the pairs (\texttt{SumSCQ}, \texttt{AvgIDF}) or (\texttt{SumSCQ}, \texttt{AvgVAR}) are observed to be negative ($\rho <-0.3$).
Furthermore, the post-retrieval predictors exhibit a significant reliance on the amount of training data, which leads to low correlations in collections with fewer training samples.


% A similar pattern appears in CW09B, where \texttt{AvP} and \texttt{AvNP} are negatively correlated with \texttt{SumSCQ}. However, for TREC 678 queries, we observe no significant negative correlations among predictors, which we attribute as one reason why combining pre-retrieval QPP approaches does not enhance performance and may even reduce it.
% \inote{nicher puro ta rewrite korte hobe.}

By integrating the findings from the heatmap in Figure~\ref{fig:heatmap} with the fused predictors presented in Tables~\ref{tab:pre-ret-combined-table} and~\ref{tab:post-ret-combined-table}, we propose the following three hypotheses.

\begin{hyp}[H\ref{hyp:first}] \label{hyp:first}
If the correlation between predictors is moderate to high, combining them will not significantly improve performance.
\end{hyp}

Based on this hypothesis, we can analyze the results in the tables, particularly for pre-retrieval in TREC Robust and post-retrieval in CW09B, to understand the lack of improvement in the combined predictors.
Despite observing an overall above-average correlation between the predictors in these two cases (the first and fifth heatmaps in Figure~\ref{fig:heatmap}), the combined results for TREC Robust (in Table~\ref{tab:pre-ret-combined-table}) and CW09B (in Table~\ref{tab:post-ret-combined-table}) do not yield any improvements.


% \inote{Robust-pre ar CW09B-post}

\begin{hyp}[H\ref{hyp:second}] \label{hyp:second}
Low correlation among predictors may lead to an improvement in performance when they are combined.
\end{hyp}
% \inote{Robust-post ar DL-post}

In the fourth and sixth heatmaps in Figure~\ref{fig:heatmap}, we observe lower correlations among the pairs of post-retrieval predictors for the Robust and DL collections.
Our hypothesis suggests that in such cases, combining predictors could enhance performance.
This is supported by the results in Table~\ref{tab:post-ret-combined-table}, where we note improvements in these two collections.



\begin{hyp}[H\ref{hyp:third}] \label{hyp:third}
 If the correlation between predictors is negative, combining them may degrade performance.
\end{hyp}
% \inote{CW09B-pre ar DL-pre}

When the pre-retrieval predictors are applied to the TREC DL collection, we observe significant negative correlations between pairs of predictors.
Our third hypothesis, \textbf{H3}, posits that combining predictors of these types, that conflict with one another may degrade overall performance.
This is empirically verified in Table~\ref{tab:pre-ret-combined-table} for the DL dataset, where all metrics against the combined predictors indicate a decline in performance.



Thus, in response to \textbf{RQ-3}, we conclude that a discernible relationship, whether positive or otherwise, among the predictors is evident due to which they exhibit similar performance producing the observed correlations.
This is supported by the heatmap and result tables, and is formalized by the proposed hypotheses.


% Interestingly, when comparing pre and post QP predictors, we find that \texttt{MaxIDF} and \texttt{AvgIDF}, despite their simplicity, perform similarly to unsupervised post-retrieval approaches in terms of \emph{RMSE} across the three datasets. In CW09B, \texttt{MaxIDF} even performs comparably to neural QPP approaches with respect to \emph{sMARE}.
%of \texttt{MaxIDF} is even comparable to neural QPP approaches in terms of \emph{sMARE}. 



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> ecir25/figs/heatmap_pre_post.tex <==
\begin{figure}[t]
\centering

% % OLD
% % pre vs. post
% \includegraphics[width=.35\textwidth]{figs/robust_pre_post.pdf}
% \includegraphics[width=.277\textwidth]{figs/cw09_pre_post.pdf}
% \includegraphics[width=.346\textwidth]{figs/dl_pre_post.pdf}

\includegraphics[width=.342\textwidth]{figs/heatmap/pre_post_pearsons_RB.pdf}
\includegraphics[width=.275\textwidth]{figs/heatmap/pre_post_pearsons_CW.pdf}
\includegraphics[width=.358\textwidth]{figs/heatmap/pre_post_pearsons_DL.pdf}
\caption{
\small
Heatmap visualizing the rank correlation among the pre-retrieval and post-retrieval QPP methods based on their individual QPP scores. 
Colour intensity represents the correlation values between the corresponding techniques measured with $\rho$. 
% The comparison is presented for TREC Robust, CW09B and TREC DL, respectively (from left to right).
\label{fig:heatmap_pre_post}
}

\end{figure}



==> ecir25/fusion-techniques.tex <==
%\section{Fusion}\label{fusion}

%\inote{baad}

%We use standard Fusion-based approaches to combine different QPP approaches. These are categorized into two groups: i) score-based methods, and ii) rank-based methods. 

%1. CombMAX($d$)

%2. CombMin($d$)

%3. CombSUM($d$)

%4. CombMNZ ($d$)

%5. Borda fuse 

%6. Condorcet

%7. Reciprocal Rank Fusion (RRF) 




%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "main"
%%% End:


==> ecir25/intro.tex <==
\section{Introduction}\label{sec:intro}

Query Performance Prediction (QPP) has long been an important area of study within information retrieval (IR)~\cite{carmel_sigir10,townsend_2002_clarity,precision_prediction,survey_preret_qpp,kurland_unified_2011,qpp_ref_list_sigir17,uef_kurland_sigir10,kurland_tois12,zhou:2006,zhou_2007_qpp}. QPP focuses on estimating (without utilizing relevance judgments) how well a search engine will perform on a given query. 
Accurate predictions of query performance can guide decisions regarding search strategies, resource allocation, and query reformulation~\cite{Feild,Li:2012,RhaSB17,querysuggestion}. 
Over the years, various QPP approaches have been proposed \cite{townsend_2002_clarity,qpp_preret_ecir08,banerjee03extendedgloss,rada:avpath,patwardhan:avvp,qpp_coherence,mothe_linguistics,amati_2004_difficulty,townsend_2004_drift,carmel_2006_what,zhou_2007_qpp,shtok_qpp_ref_list,qpp_ref_list_sigir17,kurland_tois12}. These methods can be broadly categorized as pre-retrieval or post-retrieval techniques. 
Pre-retrieval methods~\cite{survey_preret_qpp,qpp_preret_springer,qpp_preret_ecir08} estimate query difficulty using only the query and collection statistics, while post-retrieval methods~\cite{townsend_2002_clarity,kurland_tois12,zhou_2007_qpp,uef_kurland_sigir10,roitman_scnqc,qpp_ref_list_sigir17,shtok_qpp_ref_list} also use retrieval results (ranked lists of documents) to make predictions.

Given the plethora of methods proposed in the literature, researchers have also investigated whether combining different QPP methods yields better predictions~\cite{vinay:2006,zhou_2007_qpp,hauff2009combination,uef_kurland_sigir10,kurland_unified_2011,kurland_back_2012}.
In a comprehensive study involving 19 pre-retrieval predictors (but no post-retrieval methods) and 3 test collections, {Hauff et al.}~\cite{hauff2009combination} showed that combining predictors yields significant improvements in correlation between predicted and actual performance. 
However, observed gains in terms of Root Mean Squared Error (\emph{RMSE}) were modest, or even non-existent. 
Based on these observations, they proposed two important guidelines regarding QPP evaluation.
\begin{enumerate}[~i)]
% \begin{enumerate}[leftmargin=*]
\item When reporting the correlation\footnote{In general discussions, we abuse notation, and use $\rho$ as an abbreviation for any of the correlation coefficients (Pearson's or Spearman's Rho and Kendall's Tau) that are commonly used when evaluating QPP methods. 
In Sections~\ref{sec:exp} and~\ref{sec:analysis} (Experimental setup, results and analysis), $\rho$ and $\tau$ are used in accordance with standard convention.} between predictions and actual performance, a 95\% confidence interval for the observed correlation should also be reported.
This helps in assessing whether observed differences between methods are statistically significant.
\item In addition to $\rho$, a listwise metric, the Squared Error (SE) between the predicted and measured retrieval effectiveness should be used as a more interpretable, pointwise metric for QPP performance, with \emph{RMSE} representing the aggregation of these values across a test collection.
\end{enumerate}

In the 15 years since the study by {Hauff et al.}, QPP has witnessed a great deal of research activity. 
Our study revisits QPP method fusion in the
light of these advancements, assessing whether the original observations generalize to newer QPP methods, evaluation metrics, and larger, more modern datasets. 
The specific directions along which the scope
of our experiments have been expanded are listed below.
\begin{itemize}
\item \textbf{Incorporation of post-retrieval methods:} While {Hauff et al.}
  limited their analysis to pre-retrieval methods, we also consider
  post-retrieval methods. These include not only traditional, unsupervised
  methods, but also newer, supervised neural approaches.
  % providing a broader picture of the effectiveness of QPPs together with
  % their combinations.
\item \textbf{Evaluation metrics:} For measuring prediction quality, we use
  \emph{scaled Mean Absolute Rank Error}
  (\emph{sMARE})~\cite{qpp_new_eval_ecir21}, in addition to the conventional
  correlation measures and \emph{RMSE}. \emph{sMARE} is a pointwise metric that is seeing
  increased use in recent QPP research. One advantage of \emph{sMARE} over \emph{RMSE} is
  that, calculating \emph{RMSE} involves fitting a regression model, since QPP
  scores are generally not intended to be interpreted as predicted values
  of standard metrics like Average Precision (AP), and are often not even in the $[0,1]$ range;
  in contrast, \emph{sMARE} is parameter free.
\item \textbf{Test collections:} {Hauff et al.} used one news collection
  (TREC 678) and two web collections (WT10G and Gov2) for their experiments.
  In our study, we repeat their experiments on the TREC 678 collection
  (also reporting figures on the Robust collection with 100 more queries),
  and extend the evaluation to ClueWeb09B, a much larger Web collection, as
  well as the more modern TREC DL/MS MARCO collections, thus providing a more comprehensive evaluation.
\end{itemize}
Therefore, our study has elements of both reproducibility (different team,
same experimental setup) and replicability (different team, different
experimental
setup)\footnote{\scriptsize\url{https://www.acm.org/publications/policies/artifact-review-and-badging-current}}.
Given that the original experiments that we seek to reproduce and extend
are 15 years old, we have not attempted to quantitatively evaluate our
efforts using recently proposed
tools~\cite{breuer2020measure,maistro2023depth}. Instead, we simply provide
here a summary of our observations that are consistent with, or differ from,
those in~\cite{hauff2009combination}.
% ``Reproducibility is critical for establishing reliable, referenceable and
% extensible research for the future.''
% Reproducibility track at at ECIR since 2015, SIGIR since 2022.

\itodo{Results + Analysis section final hoe gele eikhane ekta summary dite
  hobe.}

Additionally, we address the following research questions in this paper:
\input{rq}

% \inote{eta ki misplaced?}
% \textbf{Correlations between QPP methods:} \textsc{Hauff et al.}
% noted that many pre-retrieval methods exhibit high correlation with one
% another. 

% Our findings indicate that simple pre-retrieval methods like MaxIDF and
% AvgIDF often outperform unsupervised post-retrieval methods and perform at
% par with expensive supervised neural approaches. This raises interesting
% questions about the trade-offs between simplicity, performance, and
% reproducibility.

% Ch. neural method propose kora paper gulo ki MaxIDF/AvgIDF report kore ni? \textcolor{red}{na..first neural model holo neuralqpp~\cite{neuralqpp}. ote porishkar bole diyechhe j jehetu amra jani j so far proposed post method gulo outperform all pre-s, tai amra shudhu post gulo kei baseline hishebe nichhi}
% \textcolor{blue}{tahole ki amra ar ekta attempt nebo? je: \emph{Although researchers have suggested that post-retrieval methods are superior to pre-retrieval models, the literature still lacks a thorough comparison based on newer evaluation criteria. In this paper, we will present our initial findings in this area as well.}}

A GitHub
repository\footnote{\scriptsize\url{https://anonymous.4open.science/r/qpp-comb-2F03/}}
provides the artifacts (retrieval results / ranked lists, code for QPP
methods, fusion, and subsequent analysis) necessary for other researchers
to independently corroborate our findings.

% \item (??) In addition to the penalised regression methods considered in
% \cite{hauff2009combination}, we also look at pairwise combinations of QPP
% methods using standard fusion techniques like CombSUM, Condorcet, Borda
% count to get a better understanding of which are independent etc.??


%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "main"
%%% End:


==> ecir25/mm-tmp.tex <==
\para{Reproducibility results}%
We start by reporting our results on TREC678 in
Table~\label{tab:pre-ret-reprod-table}. Since the very same collection was
also used in \cite{hauff2009combination}, this table serves as a validation
check for our experiments. We note that our $\rho$ values are generally higher
than those reported by \textsc{hauff et al.}. Following their suggestion,
we include the 95\% confidence interval (CI) for the observed $\rho$ values.
For two predictors (\texttt{AvP}, \texttt{AvNP}), the CIs (highlighted) are
non-overlapping; since the corresponding $\rho$s are fairly low on an absolute
scale, we have not looked more carefully into this difference. For
\texttt{AvgSCQ} the difference (underlined) appears numerically
substantial, but is not, in fact, statistically significant. Of greater
concern is the noticeable difference in $\rho$ for \texttt{AvgIDF} (also
highlighted), though, strictly speaking, the corresponding CIs do overlap.
Additionally, the RMSE values that we obtain are all very close to those
reported in \cite{hauff2009combination}. We are able to conclude,
therefore, that the high-level summary of the results in
Table~\label{tab:pre-ret-reprod-table} (that \texttt{MaxIDF},
\texttt{AvgIDF}, \texttt{AvgVAR} and \texttt{MaxVAR} provide the best
predictions, both in terms of $\rho$ and \emph{RMSE}) matches the findings
reported by \textsc{hauff et al.}.

\textcolor{red}{Alternative summary of results in Table 2:}

The results for TREC-DL also clearly match the observation above:
\texttt{MaxIDF}, \texttt{AvgIDF}, \texttt{MaxVAR}, and \texttt{AvgVAR}
appear to be decidedly the best performing predictors in terms of all
metrics. This observation mostly holds for TREC-Robust as well, where
\texttt{MaxSCQ} also emerges as a promising measure, outperforming
\texttt{MaxIDF} and \texttt{AvgIDF} on two of the four metrics. ClueWeb09B
presents the most confusing picture: there is little variation in the
\emph{RMSE} values across all methods; to a lesser extent, the same holds true
for \emph{sMARE}. Overall, \texttt{MaxSCQ} does well once again; however,
the \texttt{IDF} and \texttt{VAR} variants also perform reasonably well.





%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "main"
%%% End:


==> ecir25/rq.tex <==
\begin{itemize}
\setlength{\leftmargin}{2cm} % Adjust the value as needed
    \item[\textbf{RQ1 - }] 
% \noindent\para{- RQ-1}
Does the combination of pre-retrieval QPP methods consistently enhance correlation with Average Precision (\emph{AP}) across different datasets, including recent web collections, as suggested in~\cite{hauff2009combination}?
% by prior research?
% Specifically, can combining predictors yield improvements in correlation coefficients as Hauff et al. reported, or do these combinations result in negligible or even decreased correlations in modern test collections?
Additionally, does the combination of predictors affect Root Mean Squared Error (\emph{RMSE}), which Hauff et al. found to remain stable, or does \emph{RMSE} similarly vary across newer datasets?

\item[\textbf{RQ2 - }]
% \noindent\para{- RQ-2}
Do post-retrieval approaches exhibit similar patterns? 
Specifically, does combining multiple post-retrieval QPP estimators yield a fused predictor that outperforms the individual post-retrieval approach?
% Does combining various post-retrieval QPP predictors result in a fused predictor that outperforms the individual post-retrieval QPP approaches \textcolor{red}{DR: check--you mean combined, right?}?
Furthermore, do the performance trends of these two types of predictors differ across datasets, and can we account for any observed differences?
% \textcolor{red}{check}

\item[\textbf{RQ3 - }]
% \noindent\para{- RQ-3}
% Are there any relation in the performance of the different predictors?
Following from the above, is there a relationship in the performance patterns of different QPP estimators, both within and between pre-retrieval and post-retrieval categories?
% \textcolor{red}{eta future work e?}Specifically, can correlations or dependencies be identified that might shed light on how these predictors complement or overlap in their effectiveness across various datasets?
\end{itemize}


==> ecir25/setup.tex <==
% We choose LM-Dir~\cite{lmdir} with parameter $\mu$ set to 1000.
% The performance of a search is computed based on the top retrieved 100 as well as 1000 documents.


==> ecir25/tabdefs/post-ret.tex <==
\begin{table}[h]
  \centering
  \caption{\small The performance comparisons of both unsupervised (top group) and supervised (bottom group) post-retrieval QPP methods across three datasets. The best performances are bold-faced.
  % We consider LM-DIR-based retrieval, and the retrieval depth $k$ is set to 100. 
  \textcolor{green}{final}}
  \label{tab:post-ret-table}
  
  \begin{adjustbox}{width=1\textwidth}
  
  \begin{tabular}{l |c c c c|c c c c|c c c c} 
  \toprule
  % \multicolumn{13}{c}{Post-Retrieval}\\\toprule
    & \multicolumn{4}{c}{TREC Robust} & \multicolumn{4}{c}{CW09B} & \multicolumn{4}{c}{TREC-DL} \\
    % \cmidrule{2-13}
    \cline{2-13}
 QPP & $\tau$   & $\rho$   & \emph{sMARE} & \emph{RMSE} & $\tau$   & $\rho$   & \emph{sMARE} & \emph{RMSE} & $\tau$ & $\rho$ & \emph{sMARE} & \emph{RMSE} \\
 % \midrule
 \cline{1-13}
 % \multicolumn{13}{c}{Setting retrieval depth to 100}\\\toprule

% NQC  & 0.4341 & 0.3571 & 0.1889      & 0.2011   & 0.2641 & 0.1998 & 0.2493     & 0.1638       & 0.3907   & 0.3326  & 0.2069   & 0.2376       \\
% WIG  & 0.3269 & 0.4180 & 0.2323      & 0.1936       & 0.2445 & 0.2725 & 0.2508  & 0.1555       & 0.3293  & 0.4584  & 0.2311           & 0.2188       \\
%  Clarity            & 0.2397 & 0.3633 & 0.2617      & 0.1974       & 0.2194 & 0.2971 & 0.2727           & 0.1538       & 0.2734  & 0.4163  & 0.2510           & 0.2242       \\
%  UEF-NQC            & 0.4181 & 0.3715 & 0.1931      & 0.2001       & \textbf{0.2745} & 0.2055 & \textbf{0.2457}           & 0.1622       & 0.3993  & 0.3756  & 0.1989           & 0.2308       \\
%  UEF-WIG            & 0.3052 & 0.4330 & 0.2382      & 0.1914       & 0.2563 & 0.0995 & 0.2500           & 0.1706       & 0.3460  & 0.4630  & 0.2253           & 0.2180       \\
%  UEF-Clarity        & 0.2055 & 0.2452 & 0.2721      & 0.2054       & 0.1524 & 0.3006 & 0.2928           & 0.1577       & 0.2820  & 0.4283  & 0.2483           & 0.2211       \\
%  NeuralQPP          & 0.4450 & 0.3393 & 0.1922      & 0.1991       & 0.2042 & 0.3131 & 0.2677           & 0.1535       & 0.4229  & 0.5626  & 0.2006          & 0.2025       \\
%  qppBERT-PL         & \textbf{0.5051} & \textbf{0.6466} & \textbf{0.1663}      & \textbf{0.1625}       & 0.2359 & \textbf{0.3504} & 0.2570           & \textbf{0.1513}       & \textbf{0.4483}  & \textbf{0.6406}  & \textbf{0.1837}           & \textbf{0.1892}       \\
%  Deep-QPP           & 0.4531 & 0.5470 & 0.1831      & 0.1769       & 0.2360 & 0.3357 & 0.2651           & 0.1522       & 0.4118  & 0.5724  & 0.2028        & 0.2005       \\
%  BERT-QPP           & 0.4886 & 0.6026 & 0.1722      & 0.1696       & 0.2283 & 0.3535 & 0.2686        & 0.1512       & 0.4586  & 0.6148  & 0.1865          & 0.1950       \\
 % \toprule
 % \multicolumn{13}{c}{Setting retrieval depth to 1000}\\
 % \toprule

NQC         & 0.3960 & 0.3315 & 0.2025 & 0.2025 & 0.2423 & 0.1783 & 0.2554 & 0.1726 & 0.3119 & 0.2463 & 0.2330 & 0.2577   \\
WIG         & 0.3163 & 0.3982 & 0.2367 & 0.1950 & 0.2624 & 0.3032 & \textbf{0.2447} & 0.1620 & 0.3295 & 0.4768 & 0.2315 & 0.2304   \\
Clarity     & 0.2632 & 0.3899 & 0.2515 & 0.1948 & 0.2244 & 0.3134 & 0.2693 & 0.1610 & 0.2796 & 0.4393 & 0.2459 & 0.2358   \\
UEF-NQC     & 0.3801 & 0.3469 & 0.2066 & 0.2015 & 0.2489 & 0.1853 & 0.2541 & 0.1711 & 0.3316 & 0.3092 & 0.2272 & 0.2505   \\
UEF-WIG     & 0.2938 & 0.4205 & 0.2430 & 0.1924 & \textbf{0.2697} & 0.1069 & 0.2467 & 0.1789 & 0.3402 & 0.4887 & 0.2279 & 0.2299   \\
UEF-Clarity & 0.2313 & 0.2962 & 0.2614 & 0.2019 & 0.1611 & 0.2881 & 0.2887 & 0.1664 & 0.2822 & 0.4560 & 0.2470 & 0.2325   \\

\cmidrule{1-13} 

NeuralQPP   & 0.4204 & 0.3165 & 0.2031 & 0.2003 & 0.1995 & 0.3054 & 0.2691 & 0.1619 & 0.3857 & 0.5287 & 0.2098 & 0.2212   \\
qppBERT-PL  & \textbf{0.4740} & \textbf{0.6396} & \textbf{0.1759} & \textbf{0.1632} & 0.2284 & \textbf{0.3553} & 0.2567 & \textbf{0.1591} & 0.3905 & \textbf{0.5939} & 0.2030 & \textbf{0.2113}   \\
Deep-QPP    & 0.4348 & 0.5598 & 0.1874 & 0.1747 & 0.2201 & 0.3332 & 0.2686 & 0.1604 & 0.3892 & 0.5492 & 0.2151 & 0.2176   \\
BERT-QPP    & 0.4656 & 0.6093 & 0.1808 & 0.1680 & 0.2233 & 0.3424 & 0.2699 & 0.1598 & \textbf{0.4111} & 0.5459 & \textbf{0.1992} & 0.2205   \\
    
\bottomrule
\end{tabular}
\end{adjustbox}  

\end{table}

==> ecir25/tabdefs/reg-post.tex <==
\begin{table}[h!]
  \centering
    \caption{\small Penalized regression results for post-retrieval methods for the three datasets. We report \emph{p-value} while comparing RMSE of the combined predictor with respect to the best-performing predictor, \texttt{qppBERT-PL} as shown in Table \ref{tab:post-ret-table}.
     \textcolor{red}{highlight the best, worst.}
    }
  \label{tab:regr-post-ret-table}

  \begin{adjustbox}{width=1\textwidth}
  
  \begin{tabular}{l|c c c c c|c c c c c|c c c c c} 
  \toprule
    % \multicolumn{16}{c}{Post-Retrieval}\\\toprule
     & \multicolumn{5}{c}{TREC Robust} & \multicolumn{5}{c}{CW09B} & \multicolumn{5}{c}{TREC-DL} \\
     \cline{2-16}
    Predictor & $\tau$ & $\rho$  & \emph{sMARE} & \emph{RMSE} & \emph{p-value} & $\tau$   & $\rho$   & \emph{sMARE} & \emph{RMSE} & \emph{p-value}  & $\tau$   & $\rho$   & \emph{sMARE} & \emph{RMSE} & \emph{p-value} \\
    % \toprule
    % \multicolumn{16}{c}{Setting depth at 100} \\
    % \toprule
    % %LASSO & 0.6197 & 0.7620 & 0.1322 & 0.1358 & 0.0445 & 0.2543 & 0.3781 & 0.2599 & 0.1494 &  0.4525 & 0.4829 & 0.6523 & 0.1775 & 0.1822 & 0.3793 \\
    % OLS & \\
    % LASSO-CV & 0.6172 & 0.7257 & 0.1331 & 0.1385 & 0.0693 & 0.2355 & 0.3540 & 0.2675 & 0.1497 & 0.4615 & 0.4947 & 0.6565 & 0.1747 & 0.1820 & 0.3792   \\
    % %Elastic Net & 0.6214 & 0.7662 & 0.1317 &  0.1349 & 0.0383 & 0.2450 & 0.3863 & 0.2663 & 0.1464 & 0.3913 & 0.5155  & 0.6903 & 0.1678 & 0.1738 & 0.2506 \\
    % E-Net-CV & 0.6171 & 0.7535 & 0.1329 & 0.1384 & 0.0672 & 0.2365 & 0.3614 & 0.2673 & 0.1489 & 0.4436 & 0.4991 & 0.6659 & 0.1730 & 0.1797 & 0.3393  \\
    % %Ridge & 0.6239 & 0.7696 & 0.1309 & 0.1339 & 0.0300 & 0.2688 & 0.4249 & 0.2584 & 0.1436 & 0.3297 & 0.5367 & 0.7251 & 0.1606 & 0.1660 & 0.1468 \\
    % Ridge-CV & 0.6110 & 0.7478 & 0.1342 & 0.1405 & 0.0848 & 0.2676 & 0.4112 & 0.2587 & 0.1456 & 0.3727 & 0.5282 & 0.7016 & 0.1635 & 0.1737 & 0.2447 \\
    % %LARS & 0.6153 & 0.7553 & 0.1333 & 0.1374 & 0.0565 & 0.2467 & 0.3888 & 0.2652 & 0.1465 & 0.3920 & 0.5042 & 0.6671 & 0.1710 & 0.1816 & 0.3445 \\
    % LARS-CV & 0.6022 & 0.7418 & 0.1375 & 0.1434 & 0.1188 & 0.2062 & 0.3194 & 0.2757 & 0.1621 & 0.4976 & 0.4804 & 0.6369 & 0.1783 & 0.1856 & 0.4375  \\
    % \midrule
    % SVR & & & & 0. & 0. & & & & 0. & 0. & & & & 0.  & 0. \\
    % \toprule
    % \multicolumn{16}{c}{Setting retrieval depth at 1000} \\
    \midrule
    % \cline{1-16}
    OLS      & 0.5704 & 0.7246 & 0.1470 & 0.1469 & 0.1724 & 0.2325 & 0.3254 & 0.2610 & 0.1668 & 0.6494 & 0.4372 & 0.5946 & 0.1940 & 0.2146 & 0.5196   \\
    LASSO-CV & \textbf{0.5849} & \textbf{0.7539} & \textbf{0.1439} & \textbf{0.1378} & 0.0360 & 0.2252 & 0.3474 & 0.2669 & 0.1577 & 0.4630 & 0.4458 & 0.6183 & 0.1924 & 0.2017 & 0.3310  \\
    E-Net-CV & 0.5842 & 0.7538 & 0.1442 & 0.1379 & 0.0347 & 0.2355 & 0.3652 & 0.2646 & 0.1563 & 0.4316 & 0.4508 & 0.6266 & 0.1907 & 0.1997 & 0.2949       \\
    Ridge-CV & 0.5814 & 0.7494 & 0.1442 & 0.1396 & 0.0531 & \textbf{0.2625} & \textbf{0.4096} & \textbf{0.2582} & \textbf{0.1534} & 0.3653 & \textbf{0.4721} & \textbf{0.6553} & \textbf{0.1837} & \textbf{0.1933} & 0.2025 \\
    LARS-CV & 0.5595 & 0.7225 & 0.1512 & 0.1489 & 0.1524 & 0.1990 & 0.3073 & 0.2746 & 0.1720 & 0.5208 & 0.4471 & 0.6216 & 0.1917 & 0.2003 & 0.3032  \\
%    \midrule
%    SVR & & & & 0. & 0. & & & & 0. & 0. & & & & 0.  & 0. \\
\bottomrule
  \end{tabular}
  \end{adjustbox}
\end{table}

==> ecir25/tabdefs/reg-pre.tex <==
\begin{table}[t]
  \centering
    \caption{\small Penalized regression results for pre-retrieval methods across the three datasets. We have reported \emph{p-value} while comparing RMSE of the combined predictor with respect to the best-performing QPP method, i.e. \emph{MaxIDF} (see Table \ref{tab:pre-ret-table}) across the three datasets. \textcolor{green}{final}}
    \textcolor{red}{highlight the best, worst.}
  \label{tab:regr-pre-ret-table}

  \begin{adjustbox}{width=1\textwidth}
  
  \begin{tabular}{l | c c c c c | c c c c c | c c c c c} 
  \toprule
    % \multicolumn{16}{c}{Pre-Retrieval}\\\toprule
     & \multicolumn{5}{c}{TREC Robust} & \multicolumn{5}{c}{CW09B} & \multicolumn{5}{c}{TREC DL} \\
     \cmidrule{2-16}
     
    Predictor & $\tau$ & $\rho$  & \emph{sMARE} & \emph{RMSE} & \emph{p-value} & $\tau$   & $\rho$   & \emph{sMARE} & \emph{RMSE} & \emph{p-value}  & $\tau$   & $\rho$   & \emph{sMARE} & \emph{RMSE} & \emph{p-value} \\
    % \toprule
    %LASSO & 0.3369 & 0.4355 & 0.2229 & 0.1902 & 0.3946 & 0.1426 & 0.1427 & 0.2880 & 0.1601 & 0.5334 & 0.2993 & 0.4709 & 0.2383 & 0.2126 & 0.5992 \\
    % OLS & 0.3275 & 0.4694 & 0.2286 & 0.1897 & 0.3798 & 0.1443 & 0.1013 & 0.2869 & 0.1729 & 0.7213 & 0.2689 & 0.4296 & 0.2482 & 0.2299 & 0.8013 \\
    % LASSO-CV & 0.3212 & 0.4193 & 0.2290 & 0.1917 & 0.4244 & 0.1168 & 0.1178 & 0.2955 & 0.1590 & 0.5117 & 0.2979 & 0.4560 & 0.2384 & 0.2151 & 0.6386 \\
    % %Elastic Net & 0.3327 & 0.4379 & 0.2244 & 0.1886 & 0.3496 & 0.1371 & 0.1355 & 0.2907 & 0.1582 & 0.4963 & 0.3062 & 0.4808 & 0.2363 & 0.2104 & 0.5587  \\
    % E-Net-CV & 0.3289 & 0.4239 & 0.2263 & 0.1913 & 0.4164 & 0.1135 & 0.1153 & 0.2963 & 0.1590 & 0.5100 & 0.2972 & 0.4583 & 0.2387 & 0.2147 & 0.6305 \\
    % %Ridge & 0.3400 & 0.4495 & 0.2222 & 0.1872 & 0.3180 & 0.1434 & 0.1526 & 0.2880 & 0.1579 & 0.4886 & 0.2890 & 0.4548 & 0.2408 & 0.2136 & 0.6125 \\
    % Ridge-CV & 0.3354 & 0.4124 & 0.2243 & 0.1921 & 0.4357 & 0.1469 & 0.1540 & 0.2871 & 0.1583 & 0.4968 & 0.2866 & 0.4405 & 0.2417 & 0.2175 & 0.6752   \\
    % %LARS & 0.3168 & 0.4231 & 0.2300 & 0.1918 & 0.4101 & 0.1342 & 0.1345 & 0.2899 & 0.1602 & 0.5364 & 0.2932 & 0.4661 & 0.2401 & 0.2135 & 0.6045 \\
    % LARS-CV & 0.3051 & 0.3992 & 0.2344 & 0.1928 & 0.4495 & 0.1092 & 0.1140 & 0.2952 & 0.1588 & 0.5064 & 0.2938 & 0.4595 & 0.2393 & 0.2145 & 0.6217   \\
    % \midrule
    % SVR & 0. & 0. & 0. & 0. & 0.  & 0. \\
    % \midrule
    % \multicolumn{16}{c}{Setting the retrieval depth at 1000}\\
    \midrule
    OLS & \textbf{0.3389} & \textbf{0.4746} & \textbf{0.2250} & \textbf{0.1889} & 0.3606 & \textbf{0.1532} & 0.1304 & \textbf{0.2857} & 0.1789 & 0.7048 & 0.2009 & 0.3158 & 0.2694 & 0.2607 & 0.8959 \\
    LASSO-CV & 0.3209 & 0.4146 & 0.2309 & 0.1923 & 0.4376 & 0.1244 & 0.1471 & 0.2936 & 0.1662 & 0.4946 & 0.2471 & 0.3761 & 0.2533 & 0.2393 & 0.6871  \\
    E-Net-CV & 0.3276 & 0.4226 & 0.2289 & 0.1912 & 0.4096 & 0.1307 & 0.1517 & 0.2923 & 0.1661 & 0.4921 & 0.2492 & 0.3766 & \textbf{0.2524} & 0.2391 & 0.6832  \\
    Ridge-CV & 0.3383 & 0.4229 & 0.2253 & 0.1910 & 0.4040 & 0.1512 & \textbf{0.1763} & 0.2867 & \textbf{0.1657} & 0.4833 & 0.2405 & 0.3540 & 0.2561 & 0.2416 & 0.7324     \\
    LARS-CV & 0.2997 & 0.3851 & 0.2385 & 0.1959 & 0.5049 & 0.1141 & 0.1403 & 0.2955 & 0.1665 & 0.5002 & \textbf{0.2524} & \textbf{0.3876} & 0.2529 & \textbf{0.2387} & 0.6779 \\

\bottomrule
  \end{tabular}
  \end{adjustbox}
\end{table}
